MFuseNet: Robust Depth Estimation with Learned Multiscopic Fusion

We design a multiscopic vision system that utilizes a low-cost monocular RGB camera to acquire accurate depth estimation. Unlike multi-view stereo with images captured at unconstrained camera poses, the proposed system controls the motion of a camera to capture a sequence of images in horizontally or vertically aligned positions with the same parallax. In this system, we propose a new heuristic method and a robust learning-based method to fuse multiple cost volumes between the reference image and its surrounding images. To obtain training data, we build a synthetic dataset with multiscopic images. The experiments on the real-world Middlebury dataset and real robot demonstration show that our multiscopic vision system outperforms traditional two-frame stereo matching methods in depth estimation. Our code and dataset are available at https://sites.google.com/view/multiscopic.

==> includes/stereo.tex <==
% !TEX root =  ../main.tex

\section{STEREO MATCHING BACKGROUND}
\label{sec:stereo}

%In this section, we first introduce how our system works and actively captures stereo image pair and then present the details of the stereo matching algorithms we use.
We start illustrating how active perception can work for stereo matching with a monocular camera and present stereo matching algorithms related to our multiscopic vision system.

\subsection{Active Stereo Perception}

%Our multiscopic system is able to capture many frames which work together to reconstruct the 3D scene. If we only use two of these frames, it would degrade to a stereo vision problem, which we begin with to show how a monocular camera handles stereo problems.
Our multiscopic vision system is capable of capturing multiple images that are combined to reconstruct the 3D scene. If we only use two of these images, the depth estimation problem would degenerate to a stereo matching problem. We begin with how a monocular camera can be applied to stereo matching problems.

%The monocular camera is installed on the end of a robot arm. So it can move freely in 6D space. We command the robot to move the camera along the horizontal of the image plane, in which process two images are taken, as is presented in Fig.~\ref{fig:duck}. Unlike a binocular stereo camera, image pair with variable baseline can be captured in this system. So the baseline can be adjusted according to the need, and even using image pairs with different baselines to reconstruct one scene is possible, which makes it apply to various scenes. In this paper, for the sake of simplicity, only 20 mm baseline case is presented for correspondence matching algorithms comparison.
First, a monocular camera is installed on the end of a robot arm so the camera can be moved freely. Then we program the robot to move the camera along the horizontal axis of the image plane and two images are taken, as shown in Fig.~\ref{fig:duck}. Unlike a binocular stereo camera, the image pairs can be captured with arbitrary baselines in this active perception system. Different baselines can be applied for different purposes: accurate depth estimation of distant objects may require large baselines while stereo matching is easier with smaller baselines (less occlusion and smaller disparity).

\begin{figure}[]
\centering
\begin{subfigure}{0.45\columnwidth}
  \includegraphics[width=1\columnwidth, trim={2cm 1cm 4cm 1cm}, clip]{figures/duck/duck3}
  \caption{Left image}
  \label{fig:duck3}
\end{subfigure}
\begin{subfigure}{0.45\columnwidth}
  \includegraphics[width=1\columnwidth, trim={2cm 1cm 4cm 1cm}, clip]{figures/duck/duck2}
  \caption{Right image}
  \label{fig:duck2}
\end{subfigure}
\caption{A stereo image pair captured using the proposed active perception system. The baseline between these two images is 20 mm.}
\label{fig:duck}
\vspace{-0.3cm}
\end{figure}

Researchers have proposed several classic stereo matching methods such as the naive block matching, dynamic programming \cite{forstmann2004real}, semi-global matching \cite{hirschmuller2008stereo}, belief propagation \cite{sun2003stereo}, graph cuts \cite{kolmogorov2014kolmogorov} , and matching with convolutional neural networks \cite{zbontar2016stereo}. Specifically, we study the naive block matching method (BM), the graph cut method (GC), and the deep learning-based method (MC-CNN) \cite{zbontar2016stereo}.%, among which we include in this paper a naive block matching method, which can show the multiscopic effects straightforwardly, and a Graph Cuts method, which yields the best result.


\subsection{Block Matching}

Naive block matching is a simple and straightforward stereo matching method. This method minimizes the matching error between two blocks in the left image and the right image. To find the most similar block, we need to check all possible blocks in the same row from the minimum disparity to the maximum allowable disparity. The sum of absolute difference (SAD) is often used to measure the similarity between two blocks. For a pixel $(u, v)$ in the left image, its SAD cost with block size $2\rho+1$ and  disparity $d$ can be calculated as

\begin{equation}
  c_{\text{SAD}}(u, v, d)=\sum_{x=u-\rho}^{x=u+\rho}\sum_{y=v-\rho}^{y=v+\rho}|I_l(x,y) - I_r(x-d, y) |,
\end{equation}
where $c_{\text{SAD}}(u,v,d)$ is the cost at point $(u,v)$, $\rho$ is the radius of the block, $I_l(x,y)$ is the intensity of the pixel at $(x,y)$ in the left image and $I_r(x-d,y)$ denotes the intensity of pixel $(x-d,y)$ in the right image. The center
of the reference block is $(u, v)$ and the total number of pixels within this block is $(2\rho+1)^2$.

For the naive block matching algorithm, we simply apply the Winner-Take-All (WTA) strategy to select the correspondence with the lowest SAD cost. To improve the continuity of the results, we perform subpixel enhancement on the discrete disparity:
\begin{equation}
    d^s=d+\frac{c(u,v,d-1)-c(u,v,d+1)}
        {2c(u,v,d-1)+2c(u,v,d+1)-4c(u,v,d)},
\end{equation}
where $d$ is the integer disparity,  $d^s$ is the subpixel disparity, and $c$ is a cost volume such as $c_{\text{SAD}}$.

Applying the naive block matching algorithm on image pairs captured by our active perception system, we get a noisy disparity map as displayed in Fig.~\ref{fig:stereo}(a). Also, the depths on occluded regions and reflective tabletop are not reconstructed correctly.

\begin{figure}[]
\centering
\begin{subfigure}{0.49\columnwidth}
  \includegraphics[width=1\columnwidth, trim={2cm 1cm 4cm 1cm}, clip]{figures/duck/SAD2}
  \caption{Block matching}
\end{subfigure}
\begin{subfigure}{0.49\columnwidth}
  \includegraphics[width=1\columnwidth, trim={2cm 1cm 4cm 1cm}, clip]{figures/duck/GC22}
  \caption{Graph cuts}
\end{subfigure}
\caption{The disparity maps obtained by two stereo matching algorithms, displayed in Jet colormap. (a) is using  naive stereo block matching and (b) is using stereo graph cuts. Note that the disparities on occluded regions are not estimated accurately, and the stereo matching on the metal tabletop is not accurate due to reflection.}
\label{fig:stereo}
\vspace{-0.3cm}
\end{figure}

\subsection{Graph Cuts}

Graph cuts is one of the most popular global optimization methods for stereo matching. It is a process that assigns a label (i.e., disparity) to each pixel in the reference image such that the energy is minimized. Both our stereo graph cuts and multiscopic graph cuts are based on Graph Cuts stereo matching algorithm by Kolmogorov and Zabih \cite{kolmogorov2014kolmogorov}.

In our graph cuts optimization, the energy is composed of 4 terms defined as
\begin{equation}
  E=E_{\text{data}}+E_{\text{occlusion}}+E_{\text{smooth}}+E_{\text{unique}}.
\end{equation}

\textbf{Data term} $E_{\text{data}}$ is used to evaluate the similarity of two image patches. Note that our images may not be perfectly aligned due to the limited precision of robot arm movement, the epipolar line may deviate slightly from the horizontal or vertical direction. To compensate this, we use an improved Birchfield and Tomasi's (BT) dissimilarity for the data term \cite{birchfield1998pixel, kolmogorov2014kolmogorov}:
\begin{equation}
\begin{aligned}
  c_{\text{BT}}(u,v,d)=\max\{0, I_l(u,v)-I_r^{\min}(u-d,v), \\ I_r^{\max}(u-d,v)-I_l(u,v)\},
\end{aligned}
\end{equation}
where $I_r^{\min}$ and $I_r^{\max}$ are respectively the smallest and largest values on the subpixel neighborhood around pixel $(u-d, v)$ in the right image. For a pixel $q$ in the right image:
\begin{equation}
\begin{aligned}
  I_r^{\min}(q)=\min_\sigma\{\frac{1}{2}(I_r(q)+I_r(q+\sigma)) \},\\
  I_r^{\max}(q)=\max_\sigma\{\frac{1}{2}(I_r(q)+I_r(q+\sigma)) \},
\end{aligned}
\end{equation}
where $\sigma\in\{(0,0),(-1,0),(1,0),(0,-1),(0,1)\}$. Therefore the stereo matching for correspondence is actually performed between the half higher row and the half lower row.

\textbf{Occlusion term} $E_{\text{occlusion}}$ is used to maximize the number of matches. To encourage the disparity assignment in graph cuts optimization, any inactive pixel without assignment is penalized by energy $K$.

\textbf{Smoothness term} $E_{\text{smooth}}$ encourages to assign same disparity to adjacent pixels, especially for those with similar color. Thus if two adjacent pixels $p_1, p_2$ in left image have different disparity assignments corresponding to pixels $q_1, q_2$ in right image, a $L_1$ penalty would be added as:
\begin{equation}
\begin{split}
  V= &
  \begin{cases}
    \lambda_1 \Delta d \quad \max(|I_l(p_1)-I_l(p_2)|,\\
    \qquad \qquad \qquad
    |I_r(q_1)-I_r(q_2)|)<\theta \\
    \lambda_2 \Delta d \quad \text{otherwise}
  \end{cases}\\
  \Delta d &=\min\{|d_1-d_2|,\ d_{\text{CUTOFF}}\},
\end{split}
\end{equation}
where $\theta$ is a threshold to evaluate the color similarity, $\lambda_1, \lambda_2$ are penalty constants for similar and various pixels, $\Delta d$ is the disparity difference truncated at a threshold $d_{\text{CUTOFF}}$.

\textbf{Uniqueness term} $E_{\text{unique}}$ enforces the uniqueness of pixel correspondences. In other words, for a pixel in the left image, we do not allow two pixels in the right image match it simultaneously. This will be punished by an infinity energy $\infty$.

%With this energy $E$, the graph cuts optimization is employed and the output disparity map is displayed in Fig.~\ref{fig:stereo}(b). To suppress the discontinuous disparity transition, the input images are enlarged 4 times before the optimization. As is presented in the matching result, this map is better and there is less noise. But it still cannot handle occlusion and the reflective tabletop well.
We use the graph cuts optimization to minimize the energy $E$. To suppress the discontinuous disparity artifacts, input images are enlarged 4 times before the graph cuts optimization. As shown in Fig.~\ref{fig:stereo}(b), the resulted disparity map with graph cuts contains less noise, but artifacts on occlusion regions and the reflective tabletop still persist.

